Tit for Tattling: Cooperation, communication, and how each could stabilize the other

Indirect reciprocity is a mechanism by which individuals cooperate with those who have cooperated with others. This creates a regime in which repeated interactions are not necessary to incent cooperation (as would be required for direct reciprocity). However, indirect reciprocity creates a new problem: how do agents know who has cooperated with others? To know this, agents would need to access some form of reputation information. Perhaps there is a communication system to disseminate reputation information, but how does it remain truthful and informative? Most papers assume the existence of a truthful, forthcoming, and informative communication system; in this paper, we seek to explain how such a communication system could remain evolutionarily stable in the absence of exogenous pressures. Specifically, we present three conditions that together maintain both the truthfulness of the communication system and the prevalence of cooperation: individuals (1) use a norm that rewards the behaviors that it prescribes (an aligned norm), (2) can signal not only about the actions of other agents, but also about their truthfulness (by acting as third party observers to an interaction), and (3) make occasional mistakes, demonstrating how error can create stability by introducing diversity.

==> name.tex <==


We should separate the two distinct ways in which a deviation in action or signal could affect payoffs indirectly.
\begin{enumerate}
\item Either deviation creates a scenario in which an agent is more likely to deviate in the future, or
\item a deviation creates a scenario in which an agent will conform
\end{enumerate}

We've shown so far that deviating in one's action reduces one's action payoff, and deviating in one's signal and meta-signaling strategy reduces one's signaling payoff. But can some clever combination of deviations actually increase one's payoff -- for instance, could deviating in action strategy affect the way one signals, thereby increasing one's signal payoff? For instance, acting a certain way may trigger different types of actions from one's partner, which might lead one to signal differently than they would have). The answer, however, is no. 

\begin{enumerate}
\item Define $C_\text{signal}$ as the cost (payoff difference relative to stern discriminators) as a result of one's signal, and $C_\text{action}$ the payoff difference as the cost as a result of one's action. We would like to show that $C_\text{signal} + C_\text{action} > 0$, that is, the combined effect of any deviation on one's signals and actions will produce a payoff decrease: a positive cost.

\item Conforming in signal produces the lowest possible first-order cost ($0$) while producing the highest possible second-order benefit, $(1 - 2\epsilon')\beta$ (equal to the difference between being cooperated with every time and being defected with every time, modulo error). Because the conforming signal strategy produces the lowest-cost, highest-benefit situation, any deviation in signal can only hurt, that is $C_\text{signal} \geq 0$.

\item Because $C_\text{signal} \geq 0$, it will suffice to show that $C_\text{action} > 0$.
\item The only way to change one's action payoff is through changing one's action strategy [FIG **]. But we've already shown that any changes to one's action strategy reduce one's action payoff, so $C_\text{action} > 0$. 
\end{enumerate}
We conclude that any deviations in strategy will lead to strictly lower payoffs.


Under these assumptions, what might we delineate as the `relevant' world state? For actors, probably only their own tag and their partner's tag. For signalers, their own tag and action, and those of their partner. For meta-signalers, they might make use of the actions of the actors they are observing, the full chain of signals leading up to their own (recall that observers might be located in a chain), and perhaps their own tag, and that of their observee. 

In the case of actors, the world state is defined only by two parameters, so any possible world state is reasonably likely to occur with minimal error pileup. In the case of signaling and meta-signaling, more parameters define the world state. However, it is still true that if we assume a very large number of interactions per generation, all configurations are likely to happen sooner or later. 
